Enhanced Sliding Window Superposition Coding for Industrial Automation

The introduction of 5G has changed the wireless communication industry. Whereas previous generations of cellular technology are mainly based on communication for people, the wireless industry is discovering that 5G may be an era of communications that is mainly focused on machine-to-machine communication. The application of Ultra Reliable Low Latency Communication in factory automation is an area of great interest as it unlocks potential applications that traditional wired communications did not allow. In particular, the decrease in the inter-device distance has led to the discussion of coding schemes for these interference-filled channels. To meet the latency and accuracy requirements of URLLC, Non-orthogonal multiple access has been proposed but it comes with associated challenges. In order to combat the issue of interference, an enhanced version of Sliding window superposition coding has been proposed as a method of coding that yields performance gains in scenarios with high interference. This paper examines the abilities of this coding scheme in a broadcast network in 5G to evaluate its robustness in situations where interference is treated as noise in a factory automation setting. This work shows improvements of enhanced sliding window superposition coding over benchmark protocols in the high-reliability requirement regions of block error rates $\approx 10^{-6}$.

==> temp.tex <==


\subsection{Code Rate}
The coding rate is important to the overall success rate of each code as it changes the error correcting capabilities of the ECC. By varying the code rate of the simulation, it can be observed that the performance of ESWSC and SWSC will be better than those presented by both standard coding methods. The SWSC and ESWSC are able to reach the channel capacity at a lower coding rate when compared to the MLC methods when we set the SNR value of the simulation to be 14dB.
\begin{figure}[H]
\centerline{\includegraphics[scale=0.75]{OG.png}}
\caption{Coding Rate}
\label{fig: Coding Rate}
\end{figure}


Rate					450	0.99956	0.99988	0.99896	0.99928
									
456	0.84728	0.96672	0.83436	0.84996	456	0.99908	0.9996	0.99948	0.99924
									
458	0.8292	0.96448	0.82496	0.8514	458	0.99924	0.99964	0.99948	0.99952
									
460	0.81228	0.9712	0.8394	0.84588	460	0.9996	0.99968	0.99968	0.99976
									
462	0.84236	0.96512	0.83276	0.83452	462	0.99932	0.99964	0.99932	0.99928
									
464	0.79224	0.96292	0.82764	0.84556	464	0.99936	0.99968	0.99948	0.9992

